Neural Graph Evolution: Towards Efficient Automatic Robot Design

Despite the recent successes in robotic locomotion control, the design of robot relies heavily on human engineering. Automatic robot design has been a long studied subject, but the recent progress has been slowed due to the large combinatorial search space and the difficulty in evaluating the found candidates. To address the two challenges, we formulate automatic robot design as a graph search problem and perform evolution search in graph space. We propose Neural Graph Evolution (NGE), which performs selection on current candidates and evolves new ones iteratively. Different from previous approaches, NGE uses graph neural networks to parameterize the control policies, which reduces evaluation cost on new candidates with the help of skill transfer from previously evaluated designs. In addition, NGE applies Graph Mutation with Uncertainty (GM-UC) by incorporating model uncertainty, which reduces the search space by balancing exploration and exploitation. We show that NGE significantly outperforms previous methods by an order of magnitude. As shown in experiments, NGE is the first algorithm that can automatically discover kinematically preferred robotic graph structures, such as a fish with two symmetrical flat side-fins and a tail, or a cheetah with athletic front and back legs. Instead of using thousands of cores for weeks, NGE efficiently solves searching problem within a day on a single 64 CPU-core Amazon EC2 machine.

==> relwork.tex <==
%!TEX root = nips2018.tex

\section{Related work}
\SF{Don't we need this section??}\\
% \subsection{Evolutionary Algorithms}
{\bf Neural architecture search.} Significant attention has recently been devoted to the problem of architecture search~\cite{liu2017hierarchical,floreano2008neuroevolution,real2017large,stanley2002evolving,kitano1990designing,stanley2009hypercube, maniezzo1994genetic}.
Most of these works employ evolutionary algorithms (EA), which evaluate the fitness of the current model and evolve the topology of the architecture accordingly.
%Recently, Evolutionary algorithms (EA) have been intensively applied to the problems of architecture search of neural networks~\cite{liu2017hierarchical,floreano2008neuroevolution,real2017large,stanley2002evolving,kitano1990designing,stanley2009hypercube, maniezzo1994genetic}.
%In these papers, the authors evaluate the fitness of the current model and evolve the topology of the architecture accordingly.
For example, in~\cite{liu2017hierarchical}, hierarchical genetic representation scheme is applied during evolution.
In another line of research, reinforcement learning is used to search for the best architecture~\cite{zoph2016neural, zoph2017learning,pham2018efficient}.

%In the community of locomotion control, EA has been applied to evolve the weights of the neural network, i.e. the controller of the agents,
%while the topology structure is fixed~\cite{eiben2007parameter,fleming2002evolutionary,eiben1999parameter}.
%Due to the computation cost of EA algorithms, reinforcement learning~\cite{deepmindppo, trpo, ppo} is still preferred.
%Recently, in~\cite{salimans2017evolution,such2017deep},
%authors show that by using evolutionary strategy or genetic algorithms and using massive amount of parallelled workers,
%evolution algorithms are alternative trainig methods.
{\bf Artificial life.} Trying to evolve artificial agents is a long-studied problem with limited success. Some of pioneering work on evolving locomotion control agents in complex environment includes~\cite{steels1993artificial, mitchell1994genetic, langton1997artificial}. 
%Much attention has been paid on artificial life for a long time, yet limited successes are achieved,
%especially on the sub-problem of evolving locomotion control agents under complex environment
%from scratch~\cite{steels1993artificial, mitchell1994genetic, langton1997artificial}.
In~\cite{sims1994evolving}, the authors focus on training block creatures in simplified environments,
however the search for better topologies is under-explored.
Recently, soft robots are studied in~\cite{joachimczak2014fine}, which evolve by adding small cells connected to the old cells.
Most evolutionary robots~\cite{duff2001evolution, neri2010memetic} require heavy engineering of the initial structures,
and their evolution relies on careful human-guidance.
We emphasize that evolving locomotion-control agents in complex environments is an extremely challenging problem,
typically requiring  huge amounts of computation to evaluate the fitness of the creatures, where at the same time the topology search space is virtually infinite. 
%the almost infinite topology search space will make the problem especially challenging.
% \subsection{Reinforcement Learning}
% 1. MDP formulation for RL problems
% 2. Learning algorithms used in the problem
% Reinforcement learning (RL) has been receiving increasing amount of attention recently.
% With the growth of computation power of convolution neural network~\cite{alexnet},
% RL algorithms have been able to solve tasks that are previously considered challenging, including Atari games and GO~\cite{dqn,alphago}.
% In the model free locomotion control community, several notable progress have been made on the algorithms including the trust region methods~\cite{trpo,ppo,deepmindppo} and policy gradient method~\cite{lillicrap2015continuous, silver2014deterministic}.
% But in terms of the structure of the network, multiply-layer perception (MLP) is still most commonly used.
% Recently, authors in~\cite{WangICLR2018} proposed a structured policy network called {\nervenet}.
% By parsing the physical graph sturcture of agent, {\nervenet} is able to train policies that are transferable across agents with different topology.


